Multitask Instruction-based Prompting for Fallacy Recognition

Fallacies are used as seemingly valid arguments to support a position and persuade the audience about its validity. Recognizing fallacies is an intrinsically difficult task both for humans and machines. Moreover, a big challenge for computational models lies in the fact that fallacies are formulated differently across the datasets with differences in the input format (e.g., question-answer pair, sentence with fallacy fragment), genre (e.g., social media, dialogue, news), as well as types and number of fallacies (from 5 to 18 types per dataset). To move towards solving the fallacy recognition task, we approach these differences across datasets as multiple tasks and show how instruction-based prompting in a multitask setup based on the T5 model improves the results against approaches built for a specific dataset such as T5, BERT or GPT-3. We show the ability of this multitask prompting approach to recognize 28 unique fallacies across domains and genres and study the effect of model size and prompt choice by analyzing the per-class (i.e., fallacy type) results. Finally, we analyze the effect of annotation quality on model performance, and the feasibility of complementing this approach with external knowledge.

==> tables/prompts.tex <==
\begin{table*}[t!]
        \small
        \centering
        \begin{tabular}{ll|l|l}
        \hline \hline
        Name &Data &Prompt &Target\\
        \hline
        List &\textsc{Argotario} &Given the question and answer below, which of the following &\{fallacy\}\\ 
                        && fallacies occur in the answer: \{fallacies\}? \\
                        && Question: \{question\}\n Answer: \{answer\} \\
        \hline
        List &\textsc{Propaganda} &Given the sentence and fragment below, which of the following &\{fallacy\}\\ 
                        && fallacies occurs in the fragment: \{fallacies\}?  \\
                        && Sentence: \{sentence\} Fragment: \{fragment\} \\
        \hline
        Def &\textsc{Logic} &Given the following segment and definitions, determine which &\{fallacy\}\\ 
                        && of the fallacies defined below occurs in the segment. \\
                        && Definitions: \{definitions\} Segment: \{segment\} \\
        \hline
        Def &\textsc{Climate} &Given the segment and comment below, which of the &\{fallacy\}\\ 
        +Com                && following fallacies occurs in the segment: \{fallacies\}? \\
                        && Segment: \{segment\} Comment: \{comment\} \\
        \hline
        % Yes/No &Covid-19 & &\{fallacy\}\\ 
                        % &&  \\
        % \hline
        List &\textsc{Propaganda}   &Given the sentence below, which of the following    &Fragment: \{fragment\}\\ 
        +Frag                   &&fallacies does it have: \{fallacies\}? Sentence: \{sentence\}   &Fallacy: \{fallacy\}  \\
        \hline \hline
        \end{tabular}
        \caption{Prompts Examples. \textbf{Def}: fallacy definition included in the prompt.  \textbf{List}: fallacy types listed in the prompt. \textbf{Frag}: fallacious fragment and fallacy type are the generation targets. \textbf{Com}: fact-checker comments are included, which sometimes explain the fallacy of the segment (\textbf{Frag} and \textbf{Com} are done during training only).}
        \label{tab:prompt}
        % \textbf{Yes/No:} A question whether a particular fallacy type is in the segment.
    \end{table*}
